Formally Specifying the High-Level Behavior of LLM-Based Agents

Autonomous, goal-driven agents powered by LLMs have recently emerged as promising tools for solving challenging problems without the need for task-specific finetuned models that can be expensive to procure. Currently, the design and implementation of such agents is ad hoc, as the wide variety of tasks that LLM-based agents may be applied to naturally means there can be no one-size-fits-all approach to agent design. In this work we aim to alleviate the difficulty of designing and implementing new agents by proposing a minimalistic generation framework that simplifies the process of building agents. The framework we introduce allows the user to define desired agent behaviors in a high-level, declarative specification that is then used to construct a decoding monitor which guarantees the LLM will produce an output exhibiting the desired behavior. Our declarative approach, in which the behavior is described without concern for how it should be implemented or enforced, enables rapid design, implementation, and experimentation with different LLM-based agents. We demonstrate how the proposed framework can be used to implement recent LLM-based agents (e.g., ReACT), and show how the flexibility of our approach can be leveraged to define a new agent with more complex behavior, the Plan-Act-Summarize-Solve (PASS) agent. Lastly, we demonstrate that our method outperforms other agents on multiple popular reasoning-centric question-answering benchmarks.

==> content/discussion.tex <==
\section{Discussion}

The specification provided by the user provides a type of contract for agent behavior which can be leveraged by an LLM service provider to improve the execution of LLM-based agents. An immediate application of this is prompt validation, where the few-shot examples provided by the user can be validated against the LTL formula automatically to detect inconsistencies that could derail the underlying LLM. In addition, as identified by \cite{xu2023rewoo}, tool-use requires that the LLM be suspended mid-generation to wait on the result of a tool call. However, as there is no straightforward means of signaling to an LLM provider that the decoding state should be suspended rather than terminated, most approaches (e.g., \cite{yao2022react,shinn2023reflexion}) that incorporate external tools do so by reprompting (i.e., redundantly calling the LLM on all previous outputs concatenated with the tool result). In our framework, this expensive strategy can be avoided, as all points where the LLM must suspend its state are explicitly identified in the list of state definitions. 

Beyond optimizations to decoding, our framework also gives the user much more control over LLM generation than they would have otherwise. It is trivial to impose content-based constraints on the LLM for certain states (e.g., requiring the \texttt{Action} state in ReACT to decode to only legal API names). In our implementation, we also allow the user to specify other types of constraints that are not related to content (e.g., each state may only decode a maximum number of tokens).


